Graph Neural Networks Use Graphs When They Shouldn't

Predictions over graphs play a crucial role in various domains, including social networks and medicine. Graph Neural Networks (GNNs) have emerged as the dominant approach for learning on graph data. Although a graph-structure is provided as input to the GNN, in some cases the best solution can be obtained by ignoring it. While GNNs have the ability to ignore the graph- structure in such cases, it is not clear that they will. In this work, we show that GNNs actually tend to overfit the given graph-structure. Namely, they use it even when a better solution can be obtained by ignoring it. We analyze the implicit bias of gradient-descent learning of GNNs and prove that when the ground truth function does not use the graphs, GNNs are not guaranteed to learn a solution that ignores the graph, even with infinite data. We examine this phenomenon with respect to different graph distributions and find that regular graphs are more robust to this over-fitting. We also prove that within the family of regular graphs, GNNs are guaranteed to extrapolate when learning with gradient descent. Finally, based on our empirical and theoretical findings, we demonstrate on real-data how regular graphs can be leveraged to reduce graph overfitting and enhance performance.

==> checklist.tex <==
\begin{enumerate}


 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [Yes]
   \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [Not Applicable]
   \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [Yes]
 \end{enumerate}


 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. [Yes]
   \item Complete proofs of all theoretical results. [Yes]
   \item Clear explanations of any assumptions. [Yes]     
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [Yes]
   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [Yes]
         \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [Yes]
         \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [Yes]
 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
   \item Citations of the creator If your work uses existing assets. [Yes]
   \item The license information of the assets, if applicable. [Yes]
   \item New assets either in the supplemental material or as a URL, if applicable. [Yes]
   \item Information about consent from data providers/curators. [Not Applicable]
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Not Applicable]
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. [Not Applicable]
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Not Applicable]
   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Not Applicable]
 \end{enumerate}

 \end{enumerate}

==> deprecated/implicitbias.tex <==



% \subsection{Implicit Bias of Graph Neural Networks}
In the previous section, we empirically saw that GNNs tend to overfit the graph even when they should be ignored completely. Nevertheless, we say that some graph distributions are more sensitive to this overfitting. In particular, regular graph distributions exhibit results close to that of DeepSets, which ignores the graph, and therefore seems to be robust to the topological overfitting. In this section, we theoretically analyze GNNs trained on regular graphs. We prove that when linear GNN are trained on regular graphs using GD, they converge to a unique solution that perfectly extrapolates to any regular distribution, and as a result, generalize better also in-distribution, in the overparameterized regime, with respect to other non-regular graph distributions.


Formally, we prove that when the ground truth solution is either topology-less ($\w_2^* =0$) or root-less ($\w_1^*=0$), a solution obtained by a GNN trained on $r$-regular graphs, will generalize to any $r'$-regular graphs for all $r'\neq r$:

\begin{theorem}[Extrapolation in Regular Graphs]\label{thm:ood_regular}
Let $\{G_i,y_i\}$ be a set of linearly separable graph examples drawn from $D_r$ , with binary labels. Assume that the ground truth function $f^*$ generating the labels $y_i$ can be implemented by a GNN with $\w_1^*=0$ or $\w_2^*=0$. A linear GNN that fits the data perfectly will generalize for graphs drawn from a distribution of $r'$-regular graphs, for any $r'\neq r$.
\end{theorem}

\Thmref{thm:ood_regular} states that the max-margin solution to which the GNN converges to generalizes well to regular graphs of any regularity degree. Nevertheless, it is not clear in advance that the solution space contains bad solutions that will not generalize well. We prove that not only do there always exist such solutions, but for every other solution, there exists a test data for which the model fails with an error arbitrarily large. 


\begin{theorem}[Existence of Bad Solutions]\label{thm:regular_bad_solutions}
Let $\{G_i,y_i\}$ be a set of $r$-regular graph examples drawn from $D_r$ , with binary labels. There exist bad solutions $\w'$ that will produce an arbitrarily large error on $r'$-regular graphs. 
% Moreover, all solutions except the max-margin solution, are bad solutions.
\end{theorem}



% \input{generalization.tex}

% Our theoreticsults use the following theorem from ~\cite{NEURIPS2018_0e98aeeb} on the implicit bias of homogeneous polynomial parameterized networks:

% \begin{theorem}\label{thm:soudry}{\cite{NEURIPS2018_0e98aeeb}}
% For any homogeneous polynomial map$ P : \mathbb{R}^P \rightarrow \mathbb{R}^D$ from parameters $w \in  \mathbb{R}^D$ to linear predictors, almost all datasets $\{x_n,y_n\}_{n=1}^N$ separable by $B := \{P(w) : w \in  \mathbb{R}^P \}$, almost all initialization $w(0)$, and any bounded sequence of step sizes $\{\eta_t\}_t,$ consider the sequence of gradient descent updates $w(t)$ from eq. (7) for minimizing the empirical risk objective $LP (w)$ in (4) with exponential loss $l(u, y) = exp(-uy)$.
% If (a) the iterates $w(t)$ asymptotically minimize the objective, i.e., $\mathcal{L}_P(w(t)) = \mathcal{L}(P(w(t))) \rightarrow 0$
% (b) $w(t)$, and consequently $\beta(t) = P(w(t))$, converge in direction to yield a separator with positive
% margin, and (c) the gradients w.r.t. to the linear predictors, $\nabla_{\beta} \mathcal{L}(\beta(t))$ converge in direction, then the
% limit direction of the parameters $w^{\infty} = \lim_{t\rightarrow \infty} \frac{w(t)}{\|w\|_2}$ is a positive scaling of a first order stationary $t\rightarrow \|w(t)\|_2$
% point of the following optimization problem,
% $$\min_{w\in \mathbb{R}^D} \|w\|_2 ~~s.t.~~ \forall n, ~ y_n\langle x_n, P(w)\rangle \geq 1$$.
% \end{theorem}

% In this section, we assume an over-parameterized linear setting, with exponential loss as the loss function and gradient descent as the optimization algorithm.
% We assume sum-pooling, nevertheless, all results hold for mean-pooling with mild modifications that are discussed in the appendix.



To prove Theorem~\ref{Figure:ood_regular}, we utilize a result from ~\Thmref{thm:soudry}, which states that the implicit bias of GD when training homogeneous neural networks, converges to the max-margin solution. 
We use it to prove the following Lemma: 

\begin{lemma}[Parameters Alignment in Multiple Layers ]\label{thm:regular_multi_layers}
Let $S = \{G_i,y_i\}$ be a set of linearly separable graph examples drawn i.i.d from $D_r$ , with binary labels. An over-parameterized $L$-layers GNN with sum-pooling that fits $S$ perfectly, converges to a solution where in each layer
$\w_2^{(k)} = r\w_1^{(k)}$. In particular, the self-vector $\w_1^{(k)}$ and topology-vector in each layer $\w_2^{(k)}$ are aligned.
\end{lemma}

When a readout layer is added to the head of the network, also the final predictor components are aligned, as we state and prove in~\ref{sec:regular_with_readout}


For the sake of clarity, we present our analysis in the setting of one-layer GNNs with no readout. The results generalize for multiple layers and with readout, and these cases are deferred to the appendix.
We denote the final predictor with $f(\x,\w)$, and write it as:
\begin{equation}
\begin{aligned}
    &f(X,\w) = \sum_i^{|V|} h_i^{(2)} = \w_1\cdot \sum_i^{|V|} \x_i + \w_2\cdot \sum_{j\in N(i)} \x_j \\
    & = \w_1\cdot \sum_i^{|V|} \x_i +  \w_2\cdot \sum_i^{|V|} \sum_{j\in N(i)} \x_j 
\end{aligned}
\end{equation}\label{eq:final_predictor_general}

Then \Thmref{thm:soudry}, translated to our notation, states that a linear GNN trained with GD  will converge to the solution of the following quadratic problem:

\begin{equation}
\begin{split}
    \begin{array}{ll}
    \min & \|\w_1\|_2^2 + \|\w_2\|_2^2  \\
    s.t. & y^{(k)} \left[ \w_1 \cdot \sum_i \x_i^{(k)} + \w_2 \sum_{i} deg(v_i)^{(k)} \x_i^{(k)}\right]  \geq 1 \\
       &\forall (\x^{(k)}, y^{(k)})\in D 
    \end{array}
    \label{eq:maxmarggeneral}
    \end {split}
\end{equation}

This can be viewed as a max-margin problem in $2d$ space, where the input vector is $\left[\sum_i \x_i^{(k)}  , \sum_{i} deg(v_i)^{(k)}\x^{(k)}_i\right]$. In other words, each graph input with feature vectors(of the vertices) in $\mathbb{R}^d$ can be viewed as a vector of length $2d$ where the first $d$ coordinated are the the sum of the feature vectors over the vertices, and the last $d$ coordinated are a weighted sum of the feature vectors over the vertices, depending on the vertices' degrees.

Our goal is to derive properties on the connection of  $\w_1$ and $\w_2$, in the solution. While, formulation above holds for any graph distribution, the training distribution will of course affect the properties of the solution. 
We now turn to analyze the solution in a more specific case, where the training graph distribution is of $r$-regular graphs, i.e. graphs where all vertices share the same degree $r$, for some $r\in \mathbb{N}$.


We now turn to analyze the solution learned when trained on regular graphs.





% Our theoreticsults use the following theorem from ~\cite{NEURIPS2018_0e98aeeb} on the implicit bias of homogeneous polynomial parameterized networks:

% \begin{theorem}\label{thm:soudry}{\cite{NEURIPS2018_0e98aeeb}}
% For any homogeneous polynomial map$ P : \mathbb{R}^P \rightarrow \mathbb{R}^D$ from parameters $w \in  \mathbb{R}^D$ to linear predictors, almost all datasets $\{x_n,y_n\}_{n=1}^N$ separable by $B := \{P(w) : w \in  \mathbb{R}^P \}$, almost all initialization $w(0)$, and any bounded sequence of step sizes $\{\eta_t\}_t,$ consider the sequence of gradient descent updates $w(t)$ from eq. (7) for minimizing the empirical risk objective $LP (w)$ in (4) with exponential loss $l(u, y) = exp(-uy)$.
% If (a) the iterates $w(t)$ asymptotically minimize the objective, i.e., $\mathcal{L}_P(w(t)) = \mathcal{L}(P(w(t))) \rightarrow 0$
% (b) $w(t)$, and consequently $\beta(t) = P(w(t))$, converge in direction to yield a separator with positive
% margin, and (c) the gradients w.r.t. to the linear predictors, $\nabla_{\beta} \mathcal{L}(\beta(t))$ converge in direction, then the
% limit direction of the parameters $w^{\infty} = \lim_{t\rightarrow \infty} \frac{w(t)}{\|w\|_2}$ is a positive scaling of a first order stationary $t\rightarrow \|w(t)\|_2$
% point of the following optimization problem,
% $$\min_{w\in \mathbb{R}^D} \|w\|_2 ~~s.t.~~ \forall n, ~ y_n\langle x_n, P(w)\rangle \geq 1$$.
% \end{theorem}

% In this section, we assume an over-parameterized linear setting, with exponential loss as the loss function and gradient descent as the optimization algorithm.
% We assume sum-pooling, nevertheless, all results hold for mean-pooling with mild modifications that are discussed in the appendix.







% Assume that the GNN is trained on $r$-regular graphs.
% In this case, the final predictor from Equation~\ref{eq:final_predictor_general} can be written as:
% \begin{equation*}
%    f(X, \w) \w_1 \cdot \sum_i^{|V|} \x_i + d \w_2 \sum_{i}^{|V|} \x_i = (\w_1 + d\w_2) \cdot \sum_{i}^{|V|} \x_i
% \end{equation*}
% Then, the max-margin problem in~\eqref{eq:maxmarggeneral} becomes:
% \begin{equation}
%     \begin{array}{ll}
%     \min_{\w_1,\w_2} & \|\w_1\|_2^2 + \|\w_2\|_2^2  \\
%     s.t. & y^{(k)} [(\w_1 + d\w_2) \cdot \sum_i \x_i^{(k)}]  \geq 1 \\ \forall (\x^{(k)},y^{(k)})\in D 
%     \end{array}
%     \label{eq:maxmargregular}
% \end{equation}
% In particular, in the case of regular graphs, although we learn two vectors $\w_1$ and $\w_2$, the model only 'cares' about their weighted sum $\tw = \w_1 + d\w_2$

% Let $D_r$ be a distribution of $r$-regular graphs. We show that GNN trained on examples drawn from $D_r$, will converge to a solution where $\w_1$ and $\w_2$ are aligned, with a scale of $r$:
% \begin{theorem}[Parameters Alignment and Norms Ratio in Regular Graphs]\label{thm:implicit_bias_regular}
% Let $S = \{G_i,y_i\}$ be a set of linearly separable graph examples drawn i.i.d from $D_r$ , with binary labels. An over-parameterized one layer GNN with sum-pooling that fits $S$ perfectly, converges to a solution $\w=[\w_1, \w_2]$ where
% $\w_2 = r\w_1$. In particular,  the root-vector $\w_1$ and topology-vector $\w_2$ are aligned.
% \end{theorem}

% The proof is based on an analysis of the KKT of the convex quadratic problem.
% It is not hard to conclude equivalent results for linear GNNs with $L$ layers. In this case, the relation $\w_2=d\w_1$ will hold for each layer separately:
% \begin{theorem}[Parameters Alignment in Multiple Layers ]\label{thm:regular_multi_layers}
% Let $S = \{G_i,y_i\}$ be a set of linearly separable graph examples drawn i.i.d from $D_r$ , with binary labels. An over-parameterized $L$-layers GNN with sum-pooling that fits $S$ perfectly, converges to a solution where in each layer
% $\w_2^{(k)} = r\w_1^{(k)}$. In particular, the self-vector $\w_1^{(k)}$ and topology-vector in each layer $\w_2^{(k)}$ are aligned.
% \end{theorem}

% When a readout layer is added to the head of the network, also the final predictor components are aligned, as we state and prove in~\ref{sec:regular_with_readout}


%  \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.95\linewidth]{images/regular_ratio.png}
%     \caption{The ratio between the norms of the topological weights and the root weights, during training GNNs on regular data. $V$ is the number of vertices in the graph, and $r$ is the regularity degree. Final predictor refers to the ratio between $u^TW_2$ and $u^TW_1$}
%     \label{Figure:ragular_ratio}
% \end{figure}

% \begin{theorem}[Parameters Alignment and Norms Ratio in Regular Graphs]\label{thm:implicit_bias_regular}
% Let $S = \{G_i,y_i\}$ be a set of linearly separable graph examples drawn i.i.d from $D_r$ , with binary labels. An over-parameterized one layer GNN with sum-pooling that fits $S$ perfectly, converges to a solution $\w=[\w_1, \w_2]$ where
% $\w_2 = r\w_1$. In particular,  the root-vector $\w_1$ and topology-vector $\w_2$ are aligned.
% \end{theorem}


% An immediate conclusion from Theorem~\ref{eq:maxmargregular} is that there is more norm on the topological weights than on the root weights: 
% \begin{conclusion}[Topological Norm]\label{thm:implicit_bias_regular}
% Let $S = \{G_i,y_i\}$ be a set of linearly separable non-empty graph examples drawn i.i.d from $D_r$ , with binary labels. An over-parameterized one layer GNN with sum-pooling that fits $S$ perfectly, converges to a solution $\w=[\w_1, \w_2]$ where
% $$\| w_2 \| > \|w_1\|$$.
% \end{conclusion}

% The proof is immediate as  $\w_2 =d\w_1 \implies \|\w_2\| =d\|\w_1\| $.



==> over_parameterized_gnns.tex <==


In this section, we set the notation and setting for this work. 
A graph example is a tuple $G = (A_{G}, X_{G})$. $A_{G}$ is an adjacency matrix representing the \struct of the graph. Each node $i$ is assigned with a feature vector $\x_i \in \reals^{d}$, and all the feature vectors are stacked to a feature matrix $X_{G}\in \reals^{n\times d}$, where $n$ is the number of nodes in $G$. The set of neighbors of node $i$ is denoted by $N(i)$. We denote the number of samples in a dataset by $m$.
We focus on the common class of Message-Passing Neural Networks~\cite{morris2021weisfeiler}.
In these networks, in each layer, each node updates its representation as follows:
\begin{equation}\label{eq:gnn}
    h_i^{(k)} = \sigma\left(W^{(k)}_1 h_i^{(k-1)} + W^{(k)}_2 \sum_{j\in N(i)} h_j^{(k-1)} +b^{(k)}\right)
\end{equation}
 Where $W_1^{(k)}, W_2^{(k)} \in \reals^{d_k\times d_{k-1}}$. The initial representation of node $i$ is its feature vector $h_i^{(0)} = \x_i$.
The final node representations ${h_i^{(L)}}_{i=1}^{|V|}$ can be then used for any downstream task.
We focus on graph-level tasks, where a final graph $z_{G_i}$ representation is obtained by a permutation-invariant pooling layer that combines all the final node representations. e.g. by summing them $z_{G_i} = \sum_{j=1}^{|V|} h_j^{(L)}$. $z_{G_i}$ is sometimes followed by another linear transformation called \textit{readout} that we denote by $W_3$.
We refer to $W_1^{(k)}$ as the \textit{root-weights} of layer $k$ and to $W_2^{(k)}$ as the \textit{topological-weights} of layer $k$.
One way GNNs can ignore non-informative \struct is by zeroing the topological weights $W_2^{(k)}=\bar{0}$.
% Formally, we define a \struct $A$ to be \textit{non-informative} for a graph function $f$ if $f(X, A) = f(X)$.
We note that graphs can also be empty, i.e., have no edges. In this case, the topological weights is not trained, and the GNN is equivalent to a Deepset~\cite{zaheer2018deep}. As sets(empty graphs) and Deepsets are special cases of graphs and GNNs, For the sake of simplicity, we will use the graph and GNNs terms.



% One reason why vertex-level tasks are not considered here is that in these tasks the examples are vertices, which are inherently not i.i.d as they are connected by edges that the model uses.




==> regular_extrapolation.tex <==


%  \begin{figure*}[!h]
%     \centering
%     \subfigure[]{\label{m=3}
%         \includegraphics[width=0.7\textwidth]{images/m3.png}}
% \end{figure*}
%               \begin{figure*}
%               [!ht]\ContinuedFloat
%                   \centering
%     \subfigure[]{\label{m=15}
%          \includegraphics[width=0.7\textwidth]{images/m15.png}}


% \end{figure*}
%  \begin{figure*}[!h]\ContinuedFloat
%      \centering
%     \subfigure[]{\label{star}
%         \includegraphics[width=0.7\textwidth]{images/stargraph.png}}

%     \caption{A validation of the condition in Equation 9 (appendix) on a test set of graphs drawn from (a) BA (m=3), (b) BA (m=15), (c) Star-graphs}
%     \label{Figure:extrapolation_ba}
    
% \end{figure*}
%  \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.8\linewidth]{images/stargraph.png}
%     \caption{A validation of the condition in Equation 9 (appendix) on a test set star graphs}
%     \label{Figure:extrapolation_star}
% \end{figure*}





==> tables/add_edge_synth_data.tex <==
\begin{table}[t]
  \centering
  \vskip 0.15in
      \caption{Accuracy on synthetic tasks where the original \structs{} are either informative or non-informative. In all tasks, the accuracy significantly improves with R-COV.}
    \label{table:add_edge_synth_data_exp}
\begin{tabular}{lccc}
\toprule
     &Sum&Edge&Motif\\

\midrule
Empty Graphs&97.5$\pm$0.7&50.7$\pm$1.1 &50.1$\pm$0.9\\
Original Graphs&94.5$\pm$0.9&89.9$\pm$0.7&85.0$\pm$0.6\\
\makecell{Original Graphs\\ + R-COV}&98.9$\pm$0.9&100$\pm$0.0 & 95.0$\pm$0.9\\
\bottomrule
% Reduced COV$\sim$~0.15&95.7$\pm$1.7&97.0$\pm$1.4 &90.0$\pm$0.9 \\
% Reduced COV$\sim$~0.10&97.2$\pm$1.3&99.9$\pm$ 0.3&93.0$\pm$0.5 \\
% Reduced COV$\sim$~0.05&98.9$\pm$0.9&100$\pm$0&95.0$\pm$0.9\\



\end{tabular}

\end{table}

==> tables/augmented_graph_stats_table.tex <==
\begin{table*}[t]
  \centering\fontsize{10}{11}\selectfont

\begin{tabular}{c|c|c|c|c}
     \hline
   &\#Nodes  &\#Avg \% Edges   & Mean & Std  \\

\hline
NS/Edges Original COV$\sim$0.22& 20 & 50.0& 9.48 & 2.04\\
NS/Edges Reduce COV$\sim$0.15 & 20 & 60.5 &11.50 & 1.67\\
NS/Edges Reduce COV$\sim$0.10& 20 & 72.6& 13.78 & 1.33\\
NS/Edges Reduce COV$\sim$0.05& 20 & 91.2& 17.30 & 0.82\\
Motif Original COV$\sim$0.82& 25 &&2.04 & 1.67 \\
Motif Reduce COV$\sim$0.15& 25 &&9.14 & 1.33 \\
Motif Reduce COV$\sim$0.10& 25 &&11.92 & 1.16 \\
Motif Reduce COV$\sim$0.05& 25 &&19.30 & 0.95 \\


\end{tabular}
  \caption{Statistics of the synthetic datasets we used}
    \label{table:graph_stats_augmented_table}
\end{table*}






==> tables/norms_table.tex <==
\begin{table}[t]
\centering
  \caption{Weight norms of the solutions learned by GNNs trained on graphless tasks with randomly sampled graphs. }
    \label{table:weights_norms_table}
\begin{tabular}{ccccc|}
\multicolumn{1}{c}{}  &  \multicolumn{2}{c|}{Linear} &
 \multicolumn{2}{|c}{Non-Linear}\\

     &  $\|W_1\|$ &  $\|W_2\|$  
 &  $\|W_1\|$  &  $\|W_2\|$  
\\
     \hline\\
    regular(V=50, r=5)  &1.26 &6.3  & 10.08 & 6.09 \\
    \hline
   gnp(V=20, p=0.2) & 0.11 & 1.63 &  \\
   \hline
   gnp(V=20, p=0.5) & \\
   \hline
   gnp(V=20, p=0.8) & \\
   \hline
ba(V=20, m=3) & \\
\hline
   ba(V=20, m=10) & \\
   \hline
   ba(V=20, m=15) & \\
   \hline
   star(V=20) & \\
   \hline
   full(V=20) & \\


\end{tabular}

\end{table}

==> tables/proteins_rcov.tex <==
\begin{table}[t]
 \centering
   \centering\fontsize{9}{11}\selectfont

    \caption{Proteins dataset}
     \label{table:proteins_rcov}


\begin{tabular}{ccccc}
\toprule
Original &   -20\% & -50\% & -80\% & Full \\
\midrule
58.7 ± 3.1& 61.0 ± 1.5& --& -- & --\\
\bottomrule

\end{tabular}

\end{table}

==> tables/real_data_social_exp.tex <==
\begin{table*}[t]
  \centering 
    \caption{Accuracy on real-world tasks. In all tasks, the accuracy improves with respect to the original graph as the graphs' COV is reduced.}
     \label{add_edge_real_data_exp}
\begin{tabular}{cccccc}
     &  IMDB-B& IMDB-M & COLLAB & REDDIT & REDDIT-5K
\\
\hline \\
Empty Graphs \cite{errica2022fair} & 60.7 $\pm$ 2.5& 49.1 $\pm$3.5\\

Best Accuracy from \cite{errica2022fair}  & 71.2 $\pm$ 3.9 & 48.5 $\pm$ 3.3\\

Original Graphs & 68.2 $\pm$ 2.1& 47.7  $\pm$ 0.9 \\
\hline
Original Graphs+R-COV  &74.1 $\pm$ 3.3 & 50.1 $\pm$ 3.5


\end{tabular}

\end{table*}

==> tables/real_data_with_fa_table.tex <==
\begin{table}[t]
 \centering
 

    \caption{Accuracy on real-world tasks for which results from \cite{alon2021bottleneck} are available.
    $\mathsection$ - Equation~\ref{eq:edge_weight_gnn},
    $\dagger$ - Previously reported in \cite{errica2022fair},
    $\ddagger$ - Previously reported in \cite{alon2021bottleneck}.}
     \label{with_fa}

\begin{tabular}{lcc}
\toprule
     &  Enzymes  & NCI1 
\\
\midrule

Empty Graphs$\dagger$ &  65.2 $\pm$ 6.4 & 69.8 $\pm$ 2.2 \\

Original Graphs$\dagger$ &  59.6 $\pm$ 4.5 & 80.0 $\pm$ 1.4  \\
 \makecell{Original Graphs$\dagger$\\+ FA$\ddagger$}  & \textbf{67.7 $\pm$ 5.3} &  81.5 $\pm$ 1.2  \\
Original Graphs$\mathsection$  & 58.4 $\pm$ 2.7 & 76.2  $\pm$ 1.0   \\
\makecell{Original Graphs$\mathsection$\\ + R-COV}   & 64.7 $\pm$ 3.1 & \textbf{82.6 $\pm$ 1.1} \\
\bottomrule
% Reduced COV$\sim$0.15& 74.7 $\pm$ 3.1 & 60.4 $\pm$ 3.5 & 79.0  $\pm$ 1.3 &72.4 $\pm$ 1.5 & 49.5 $\pm$ 3.1 \\

% Reduced COV$\sim$0.10&  75.9  $\pm$ 2.9 & 64.1 $\pm$ 4.8 & 82.1  $\pm$ 1.5 &73.9 $\pm$ 3.0 & 49.9 $\pm$ 2.0\\

% Reduced COV$\sim$0.05 & 76.3 $\pm$ 2.7 & 64.7 $\pm$ 3.1 & 82.6 $\pm$ 1.1 &74.1 $\pm$ 3.3 & 50.1 $\pm$ 3.5 \\


\end{tabular}

\end{table}
